Beyond Low-Pass Filters: Adaptive Feature Propagation on Graphs

Graph neural networks (GNNs) have been extensively studied for prediction tasks on graphs. As pointed out by recent studies, most GNNs assume local homophily, i.e., strong similarities in local neighborhoods. This assumption however limits the generalizability power of GNNs. To address this limitation, we propose a flexible GNN model, which is capable of handling any graphs without being restricted by their underlying homophily. At its core, this model adopts a node attention mechanism based on multiple learnable spectral filters; therefore, the aggregation scheme is learned adaptively for each graph in the spectral domain. We evaluated the proposed model on node classification tasks over eight benchmark datasets. The proposed model is shown to generalize well to both homophilic and heterophilic graphs. Further, it outperforms all state-of-the-art baselines on heterophilic graphs and performs comparably with them on homophilic graphs.

==> ASGAT - ArXiv (2)/abstract.tex <==
\begin{abstract}
Graph neural networks (GNNs) have been extensively studied for prediction tasks on graphs. As pointed out by recent studies, most GNNs assume local homophily, i.e., strong similarities in local neighborhoods. This assumption however limits the generalizability power of GNNs. %, making them incapable of handling heterophilic graphs which commonly exist in many real-world applications. 
To address this limitation, we propose a flexible GNN model, which is capable of handling any graphs without being restricted by their underlying homophily. % with different degrees of homophily.
At its core, this model adopts a node attention mechanism based on multiple learnable spectral filters; therefore, the aggregation scheme is learned adaptively for each graph in the spectral domain.
We evaluated the proposed model on node classification tasks over eight benchmark datasets. The proposed model is shown to generalize well to both homophilic and heterophilic graphs. Further, it outperforms all state-of-the-art baselines on heterophilic graphs and performs comparably with them on homophilic graphs. 

\end{abstract}



==> ASGAT - ArXiv (2)/conclusion.tex <==
m\section{Conclusion}
In this paper, we study the node classification tasks on graphs where local homophily is weak. We argue the assumption of homophily is the cause of poor performance on heterophilic graphs. In order to design more generalizable GNNs, we suggest that a more flexible and adaptive feature aggregation scheme is needed. To demonstrate, we have introduced the adaptive spectral graph attention network (\model{}) which achieves flexible feature aggregation using learnable spectral graph filters. By utilizing the full graph spectrum adaptively via the learned filters, \model{} is able to aggregate features from nodes that are close and far. For node classification tasks, \model{} outperforms all benchmarks on heterophilic graphs, and performs comparably on homophilic graphs. On homophilic graphs, \model{} also performs better for nodes with weak local homophily. Through our analysis, we find the performance gain is closely linked to the higher end of the frequency spectrum.


==> ASGAT - ArXiv (2)/experiments.tex <==
% \begin{table*}[t!]
% \begin{center}
%  \caption{Dataset statistics. We categorize the datasets into homophilic and heterophilic based on their homophily ($\beta$).}
%  \scalebox{0.8}{
%  \begin{tabular}{l l  r  r  r  r  r  r } 
%  \toprule
%  Category &Dataset & \#Nodes & \#Edges & \#Classes & \#Features & Density & $\beta$ \\
%  \midrule
%  \multirow{3}{*}{homophilic}&\cora & 2,708 & 5,429 & 7 & 1,433 & 1.44e-3 & 0.83\\
%  &\citeseer & 3,327 & 4,732 & 6 & 3,703 & 8.23e-4 & 0.71\\
%  &\pubmed & 19,717 & 44,338 & 3 & 500 & 2.28e-4 & 0.79 \\
%  \midrule
%  \multirow{4}{*}{heterophilic}&\cornell & 183 & 298 & 5 & 1,703 & 1.68e-2 & 0.11 \\
%  &\texas & 183 & 325 & 5 & 1,703 & 1.77e-2 & 0.06 \\
%  &\wisconsin & 251 & 515 & 5 & 1,703 & 1.49e-2 & 0.16\\
%  &\chameleon & 2277 & 36101 & 5 & 2,325 & 1.21e-2 & 0.25\\
%  \bottomrule
%  \end{tabular}
%  \label{table:dataset}
%  }
% \end{center}
% \end{table*}


\section{Experiments}
\label{sec:experiments}

To evaluate the performance of our proposed model, we conduct experiments on node classification tasks with homophilic graph datasets, and heterophilic graph datasets. Further ablation study highlights the importance of considering the entire spectral frequency.
%, where homophily is weak and labels of nodes represent their structural roles.

%\begin{equation}
%    \beta_v = \frac{\text{Number of $v$'s neighbors which have the same label as v}}{\text{Number of $v$'s neighbors}}\dw{.}
%        \beta_v = \frac{|\{u\in\sN_v|\ell(u)=\ell(v)\}|}{|\sN_v|}\dw{.}
%    \label{eqn:beta_v}
%\end{equation}

%\q{(need a revision)} We are interested to see how the methods perform on homophilic graph node where local homophily is weak. In terms of the learned filters, we are interested to see how they differ for homophilic and heterophilic graphs. We also plot the prediction accuracy with respect to $\beta_v$ to show how each method performs in weak homophilic neighborhoods in homophilic graphs.

% Lastly, to analyze importance of frequency bands, we carried out a ablation study by cutting out a range of frequencies iteratively. We also ablate spectral filters to analyze the necessity of using multiple heads following \citet{DBLP:conf/nips/MichelLN19}.

\subsection{Experimental Setup}


% \begin{table}[t!]
%      \centering
%      \caption{Micro-F1 results for node classification. The proposed model consistently outperforms the other variants of GNN on heterophilic graphs and performs comparably on homophilic graphs.}
%      \scalebox{0.7}{
%      \begin{tabular}{l c c c c c  c  c  c  c} 
%          \toprule
%          \\[-.7em]
%           & \multicolumn{2}{c}{\cora} & \multicolumn{2}{c}{\citeseer} & \multicolumn{2}{c}{\pubmed} & \cornell & \texas & \wisconsin \\
%          Method & Sup.& Semi.& Sup. & Semi.& Sup. & Semi. & Sup. & Sup. & Sup. \\
%          \midrule
%          Chebyshev & $88.2\pm 0.2$ & $81.1\pm0.6$ & $\textbf{79.4}\pm0.4$ & $70.0\pm0.2$ & $89.3\pm0.3$ & $77.4\pm0.8$ & $76.5\pm9.4$ & $79.7\pm5.0$& $82.5\pm2.8$\\
%          GCN & $87.4\pm 0.2$ & $82.1\pm0.6$ & $78.5\pm0.5$ & $71.5\pm0.4$ & $87.8\pm0.2$ & $79.3\pm0.4$ & $59.2\pm3.2$& $64.1\pm4.9$ & $64.1\pm6.3$\\
%          SGC & $87.2\pm0.3$ & $80.2\pm0.8$ & $78.8\pm0.4$ & $70.1\pm1.3$ & $81.1\pm0.3$ & $78.6\pm0.2$ & $58.1\pm4.6$ & $58.9\pm6.1$ & $51.8\pm5.9$\\
%          GraphSAGE & $86.3\pm 0.6$ & & $77.4\pm 0.5$ & & $89.2\pm0.5$ & & $67.3\pm6.9$ &  $82.7\pm4.8$ & $77.6\pm4.6$\\
%          ARMA & $85.2\pm2.5$ & $82.3\pm0.7$ & $76.7\pm0.5$ & $76.7\pm0.5$ & $86.3\pm5.7$ & $78.4\pm0.3$ & $74.9\pm2.9$ & $82.2\pm5.1$ & $78.4\pm4.6$\\ 
%          GAT & $87.6\pm 0.3$ & $82.8\pm0.6$ & $77.7\pm0.3$ & $71.9\pm0.7$ & $83.0\pm0.1$ & $77.4\pm0.8$ & $58.9\pm3.3$ & $60.0\pm5.7$ & $62.0\pm5.2$\\
%          APPNP & $\textbf{88.4}\pm0.3$ & $83.4\pm0.2$ & $77.6\pm0.6$ & $71.4\pm0.4$ & $86.0\pm0.3$ & $80.0\pm0.2$ & $70.3\pm9.3$ & $79.5\pm4.6$ & $81.2\pm2.5$\\
%          FastGCN & $86.1\pm 0.4$ & & $78.1\pm 0.7$ & & $86.0\pm 0.8$ & & $72.7\pm6.8$ & $68.4\pm4.6$ & $68.8\pm5.4$\\
%          ASGCN & $86.8\pm0.4$ & & $77.9\pm0.3$ & & $88.0\pm0.7$ & & $73.0\pm6.1$ & $68.1\pm7.7$ & $66.3\pm6.5$\\
%          \midrule
%          MLP & $72.1\pm1.3$ & $58.7\pm0.7$ & $74.9\pm1.8$ & $56.4\pm1.1$ & $88.6\pm0.2$ & $72.1\pm0.6$ & $80.5\pm5.8$ & $79.2\pm6.1$ & $82.7\pm4.5$\\
%          \midrule
%          \model* & $87.5\pm0.5$ & $80.7\pm0.6$ & $79.0\pm1.1$ & $70.5\pm0.7$ & $\textbf{89.9}\pm0.9$ & & $\textbf{82.7}\pm8.3$ & $\textbf{85.1}\pm5.7$ & $\textbf{85.9}\pm3.8$ \\
%          \bottomrule
%     \end{tabular}
%     }
%     \label{tab:micro_f1}
% \end{table}

% table without semisupervised learning
\begin{table*}[t!]
     \centering
     \caption{Micro-F1 results for node classification. The proposed model consistently outperforms the GNN methods on heterophilic graphs and performs comparably on homophilic graphs. Results marked with $\dagger$ are obtained from \citet{Pei2020}. Results marked with $\ddag$ are obtained from \citet{DBLP:conf/nips/ZhuYZHAK20}.}
     \scalebox{0.77}{
         \begin{tabular}{l | r  r  r | r  r  r  r r} 
             \toprule
             %\\[-.7em]
              & \multicolumn{8}{c}{$\text{Homophily} \xLeftrightarrow{\hspace*{6cm}} \text{Heterophily}$} \\
              & \multicolumn{1}{c}{\cora} & \multicolumn{1}{c}{\pubmed} & \multicolumn{1}{c|}{\citeseer} & \multicolumn{1}{c}{\chameleon} &
              \multicolumn{1}{c}{\squirrel} & \multicolumn{1}{c}{\wisconsin} & \multicolumn{1}{c}{\cornell} & \multicolumn{1}{c}{\texas} \\              
              \midrule
              \midrule
              $\beta$ & 0.83 & 0.79 & 0.71 & 0.25 & 0.22 & 0.16 & 0.11 & 0.06\\
              \#Nodes & 2,708 & 19,717 & 3,327 & 2,277 & 5,201 & 251 & 183 & 183 \\
              \#Edges & 5,429 & 44,338 & 4,732 & 36,101 & 217,073 & 515 & 298 & 325\\
              \#Features & 1,433 & 500 & 3,703 & 2,325 & 2,089 & 1,703 & 1,703 & 1,703 \\
              \#Classes & 7 & 3 & 6 & 5 & 5 & 5 & 5 & 5\\
             \midrule
             GCN & $87.4\pm 0.2$ & $87.8\pm0.2$ & $78.5\pm0.5$ & ${59.8\pm2.6}^\ddag$ & ${36.9\pm1.3}^\ddag$ & $64.1\pm6.3$ & $59.2\pm3.2$& $64.1\pm4.9$ \\
             ChevNet & $88.2\pm 0.2$ & $89.3\pm0.3$ & ${79.4}\pm0.4$  & $66.0\pm2.3$ & $39.6\pm3.0$ & $82.5\pm2.8$ & $76.5\pm9.4$ & $79.7\pm5.0$ \\
             ARMANet & $85.2\pm2.5$ & $86.3\pm5.7$ & $76.7\pm0.5$ & $62.1\pm3.6$ & $47.8\pm3.5$ & $78.4\pm4.6$ & $74.9\pm2.9$ & $82.2\pm5.1$  \\ 
             GAT & $87.6\pm 0.3$ & $83.0\pm0.1$ & $77.7\pm0.3$ & ${54.7\pm2.0}^\ddag$  & ${30.6\pm2.1}^\ddag$ & $62.0\pm5.2$ & $58.9\pm3.3$ & $60.0\pm5.7$ \\
             SGC & $87.2\pm0.3$ & $81.1\pm0.3$ & $78.8\pm0.4$ & $33.7\pm3.5$ & $46.9\pm1.7$& $51.8\pm5.9$& $58.1\pm4.6$ & $58.9\pm6.1$\\
             GraphSAGE & $86.3\pm 0.6$ & $89.2\pm0.5$ & $77.4\pm 0.5$ & $51.1\pm0.5$ & ${41.6\pm0.7}^\ddag$ & $77.6\pm4.6$ & $67.3\pm6.9$ &  $82.7\pm4.8$\\
             APPNP & $\textbf{88.4}\pm0.3$ & $86.0\pm0.3$ & $77.6\pm0.6$ & $45.3\pm1.6$ &$31.0\pm1.6$ & $81.2\pm2.5$ & $70.3\pm9.3$ & $79.5\pm4.6$\\
            %  FastGCN & $86.1\pm 0.4$ & $86.0\pm 0.8$ & $78.1\pm 0.7$ & $42.8\pm2.4$ & & $68.8\pm5.4$ & $72.7\pm6.8$ & $68.4\pm4.6$ \\
            %  ASGCN & $86.8\pm0.4$ & $88.0\pm0.7$ & $77.9\pm0.3$ & $49.5\pm1.5$ & & $66.3\pm6.5$ & $73.0\pm6.1$ & $68.1\pm7.7$ \\
             Geom-GCN & $86.3\pm0.3$ & $89.1\pm0.1$ & $\textbf{81.4}\pm0.3$ & $60.9^\dagger$ & $38.1^\dagger$ & $64.1^\dagger$ & $60.8^\dagger$ & $67.6^\dagger$ \\
             $\text{H}_2\text{GCN}$ & $88.3\pm0.3$ & $89.1\pm0.4$ & $78.4\pm0.5$ & $59.4\pm2.0$ & $37.9\pm2.0$ & $86.5\pm4.4$ & $82.2\pm6.0$ & $82.7\pm5.7$\\  
             \midrule
             MLP & $72.1\pm1.3$ & $88.6\pm0.2$ & $74.9\pm1.8$ & $45.7\pm2.7$ & $28.1\pm2.0$ & $82.7\pm4.5$ & $81.4\pm6.3$ & $79.2\pm6.1$ \\
             \midrule
             Vanilla \model{} & $-$ & $-$ & $-$ & $-$ & $-$ & $\textbf{86.9}\pm4.2$ & $\textbf{84.6}\pm5.8$ & $82.2\pm3.2$ \\ 
             \model-Cheb & $87.5\pm0.5$ & $\textbf{89.9}\pm0.9$ & $79.3\pm0.6$ & $\textbf{66.5}\pm2.8$ & $\textbf{55.8}\pm3.2$ & $86.3\pm3.7$ & $82.7\pm8.3$ & $\textbf{85.1}\pm5.7$ \\
             \model-ARMA & $87.4\pm1.1$ & $88.3\pm1.0$ & $79.2\pm1.4$ & $65.8\pm2.2$ & $51.4\pm3.2$ & $84.7\pm4.4$ & ${83.2}\pm5.5$ & $79.5\pm7.7$ \\
             \bottomrule
        \end{tabular}
    }
    \label{tab:micro_f1}
\end{table*}

\textbf{Baseline methods.~} An exact computation of \autoref{eqn:graph_wavelet_matrix} requires to compute the eigenvectors of the Laplacian matrix, which is often infeasible due to a large graph size. To overcome this issue, we approximate graph wavelet transform response of $\text{MLP}$ with Chebyshev polynomial, dubbed as \model{}-Cheb, and ARMA rational function, dubbed as \model{}-ARMA. We also report the results from the exact computation of eigenvectors whenever possible, which is dubbed as vanilla \model{}.

We compare all variants against 10 benchmark methods, they are vanilla GCN~\citep{DBLP:conf/iclr/KipfW17} and its simplified version SGC~\citep{DBLP:conf/icml/WuSZFYW19}; two spectral methods: ChevNet~\citep{DBLP:conf/nips/DefferrardBV16} and ARMANet~\citep{DBLP:journals/corr/abs-1901-01343}; the graph attention model GAT~\citep{DBLP:conf/iclr/VelickovicCCRLB18}; APPNP, which also adopts adaptive aggregation~\citep{DBLP:conf/iclr/KlicperaBG19}; the neighbourhood-sampling method GraphSage~\citep{DBLP:conf/nips/HamiltonYL17}; Geom-GCN~\citep{Pei2020} and $\text{H}_2\text{GCN}$~\citep{DBLP:conf/nips/ZhuYZHAK20}, both also target prediction on heterophilic graphs. We also include MLP in the baselines since it performs better than many GNN methods on some heterophilic graphs~\citep{Liu2020}.


\textbf{Datasets.~}We evaluate our model and the baseline methods on node classification tasks over three citation networks: \cora{}, \citeseer{} and \pubmed{}~\citep{DBLP:journals/aim/SenNBGGE08}, three webgraphs from the WebKB dataset\footnote{\url{http://www.cs.cmu.edu/afs/cs.cmu.edu/project/theo-11/www/wwkb/}}: \wisconsin, \texas{} and \cornell, and webgraphs from Wikipedia called \chameleon{} and \squirrel{}~\citep{DBLP:journals/corr/abs-1909-13021}.

To quantify the homophily of graphs, we use the metric $\beta$ introduced by \citet{Pei2020},
\begin{equation}
    \beta = \frac{1}{N}\sum_{v\in V}\beta_v\text{\; and \; }
    \beta_v = \frac{|\{u\in\sN_v|\ell(u)=\ell(v)\}|}{|\sN_v|},
\end{equation}
where $\ell(v)$ refers to the label of node $v$.
$\beta$ measures the degree of homophily of a graph, and $\beta_v$ measures the homophily of node $v$ in the graph. A graph has strong local homophily if $\beta$ is large and vice versa. Details of these datasets are summarized in \autoref{tab:micro_f1}.

\textbf{Hyper-parameter settings.~} For citation networks, we follow the experimental setup for node classification from \citep{DBLP:conf/nips/HamiltonYL17, DBLP:conf/nips/Huang0RH18, DBLP:conf/iclr/ChenMX18} and report the results averaged on 10 runs. For webgraphs, we run each model on the 10 splits provided by \citep{Pei2020} and take the average, where each split uses 60\%, 20\%, and 20\% nodes of each class for training, validation and testing, respectively. The results we report on GCN and GAT are better than \citet{Pei2020} as a result of converting the graphs to undirected before training \footnote{\url{https://openreview.net/forum?id=S1e2agrFvS}}. Geom-GCN uses node embeddings pre-trained from different embedding methods such as Isomap~\citep{Tenenbaum2000}, Poincare~\citep{Nickel2017} and struc2vec~\citep{Ribeiro2017}. We report the best micro-F1 results among all three variants for Geom-GCN.

We use the best-performing hyperparameters specified in the original papers of baseline methods. For hyperparameters not specified in the original papers, we use the parameters from \citet{DBLP:journals/corr/abs-1903-02428}. We report the test accuracy results from epochs with the smallest validation loss and highest validation accuracy. Early termination is adopted for both validation loss and accuracy, thus training is stopped when neither validation loss or accuracy improve for 100 consecutive epochs. For \model{}, we use a two-layer architecture where multi-headed filters are learned using a MLP of 2 hidden layers. Each layer of the MLP consists of a linear function and a ReLU activation. To avoid overfitting, dropout is applied in each \model{} layer on both attention weights and inputs equally. Results for vanilla \model{} are only reported for small datasets where eigen-decomposition is feasible.


\subsection{Results and Discussion}
\label{subsec:results}

%\textbf{Micro-F1}. 
We use two evaluation metrics to evaluate the performance of node classification tasks: micro-F1 and macro-F1. The results with micro-F1 are summarized in \autoref{tab:micro_f1}. Overall, on homophilic citation networks, \model{} performs comparably with the state-of-the-art methods, ranking first on \pubmed{} and second on \cora{} and \citeseer{} in terms of micro-F1 scores. On heterophilic graphs, \model{} outperforms all other methods by a margin of at least $2.4\%$ on 3 out of 4 datasets. These results indicate that \model{} generalizes well on different types of graphs. 
The results with macro-F1 are summarized in \autoref{tab:macro_f1}. Macro-F1 scores have not been reported widely in the literature yet. Here, we report the macro-F1 since the heterophilic graphs have imbalanced class distributions than the homophilic graphs. As the results show, \model{} outperforms all other methods across all heterophilic graphs in macro-F1. The difference between the two approximation methods is not significant. Except for a few cases, the difference is largely attributed to hyperparameters choices. The vanilla \model{} gives more consistent results than the approximations although the difference seems marginal.

%\textbf{Micro-F1 with respect to $\beta_v$}.

Although \model{} performs well on both homophilic and heterophilic graphs, it is unclear how \model{} performs on heterophilic neighbourhoods of an homophilic graph where nodes are mostly of different classes.
%To further investigate how our model classifies heterophilic nodes in homophilic graphs in comparison with other state-of-the-art methods, 
Thus, we report an average classification accuracy
on nodes at different levels of $\beta_v$ in \autoref{fig:noisy_neighbours} on the homophilic graphs \citeseer{} and \pubmed{}. The nodes are binned into five groups based on $\beta_v$. For example, all nodes with $0.3 < \beta_v \leq 0.4$ belong to the bin at $0.4$. We have excluded \cora{} from the report since it has very few heterophilic neighbourhoods. 


The results in \autoref{fig:noisy_neighbours} show that all models except \model{} perform poorly when $\beta_v$ is low. One may argue that the performance on heterophilic graphs might improve by stacking multiple GNN layers together to obtain information from far-distant nodes. However, it turns out that this approach introduces an oversmoothing problem~\citep{DBLP:conf/aaai/LiHW18} which actually degrades performance. On the other hand, the better performance of \model{} on heterophilic nodes suggests the adaptive spectral filters reduce noise aggregated locally while allowing far-distant nodes to be attended to. 
%\dw{(Not sure whether we need to report MV)} In addition, we plot the prediction accuracy based on majority voting (MV). MV classifies a node based on the majority class from its direct neighbors. 

%While all GNNs performs poorer on nodes of low $\beta_v$ than those of high $\beta_v$, our method consistently outperforms homophilic GNNs when $\beta_v$ is low. We argue the lack of local homophily is the reason for such difference. In order to show it, we also plot the prediction accuracy based on majority voting (MV), denoted with blue dashed lines. The rule for MV is to classify a node based on the majority class from its direct neighbors. All labels but the node to be predicted is made available in MV so MV is not a comparable benchmark but instead an indicator of how local homophily impacts GNN performance. \dw{(Can anyone guess what is happening with $\beta_v < 0.1$?)}\q{(GNAN has very good performance?)} \dw{(That's right!)} %Most GNN methods in \autoref{fig:noisy_neighbours} follow a similar pattern as MV which goes up quickly when $\beta_v$ is greater than 0.4. \model{}, on the other hand, is able to produce better accuracy when $beta_v < 0.4$.


\textbf{Attention sparsification.}
%The two variants of \model{} use two different approximation techniques for spectral filtering. For each node $v$, GNAN-T uses a threshold $t$ to eliminate low $\psi_{vu}$ (\autoref{eqn:psi}), thereby sparsifying the resulting attention matrix. However, $t$ cannot control the level of sparsification precisely. In comparison, GNAN-K keeps the $k$ largest $\phi_{vu}$ (\autoref{eqn:psi_k}); therefore
The restriction on top $k$ entries in \autoref{eqn:psi_k} guarantees a certain level of sparsification. Nonetheless, \model{} requires a partial sorting which adds an overhead of $O(n+k\log N)$. To further analyze the impact of attention sparsity on runtime, we plot the density of an attention matrix with varying $k$ in \autoref{fig:density} along with its running time. The results are drawn from two datasets: the heterophilic dataset \chameleon{} and the homophilic dataset \cora. As expected, \model{} shows a stable growth in the attention density as the value of $k$ increases. It also shows that \model{} runs much faster when attention weights are well-sparsified. In our experiments, we find the best results are achieved on $k<20$.
%We observe that the attention weights tend to converge to similar small values on all nodes when $t$ goes beyond 0.001 in both datasets. To study how efficiency is improved via sparsification, we also plot the training time averaged over 500 epochs in \autoref{fig:density}. It shows that the model \model{} runs much faster when attention weights are well-sparsified. In our experiments, we find the best results are achieved on $k<20$ for GNAN-K and $t<1e-5$ for GNAN-T. Thus, the model \model{} not only runs faster, but also performs better when attention weights are well-sparsified.

\textbf{Frequency range ablation.} To understand how adaptive spectral filters contribute to \model{}'s performance on heterophilic graphs, we conduct an ablation study on spectral frequency ranges. We first divide the entire frequency range $(0\sim2)$ into a set of predefined sub-ranges exclusively, and then manually set the filter frequency responses to zero for each sub-range at a time in order to check the impact of each sub-range on the performance of classification. By doing so, the frequencies within a selected sub-range do not contribute to neither node attention nor feature aggregation, therefore helping to reveal the importance of the sub-range. We consider three different lengths of sub-ranges, i.e., step=$1.0$, step=$0.5$, and step=$0.25$. The results of frequency ablation on the three homophilic graphs are summarized in \autoref{fig:freqency_ablation}.

The results for step=$1.0$ reveal the importance of high-frequency range $(1\sim2)$ on node classification of heterophilic graphs. The performance is significantly dropped by ablating high-frequency range on all datasets. Further investigation at the finer-level sub-ranges (step=$0.5$) shows that ablating sub-range $0.5\sim1.5$ has the most negative impact on performance, whereas the most important sub-range varies across different datasets at the finest level (step=$0.25$).
This finding matches our intuition that low-pass filters used in GNNs underlie a homophily assumption in a similar way as naive local aggregation. We suspect the choice of low-pass filters also relates to oversmoothing issues in spectral methods~\citep{DBLP:conf/aaai/LiHW18}, but we leave it for future work.


\textbf{Attention head ablation.} In \model{}, each head uses a spectral filter to produce attention weights. To delve the importance of a spectral filter, we further follow the ablation method used by \citet{DBLP:conf/nips/MichelLN19}. Specifically, we ablate one or more filters by manually setting their attention weights to zeros. We then measure the impact on performance using micro-F1. If the ablation results in a large decrease in performance, the ablated filters are considered important. We observe that all attention heads (spectral filters) in \model{} are of similar importance, and only all attention heads combined produce the best performance. Please check \autoref{sec:ablation} for the detailed results.


\begin{figure}[t!]
\centering
 \includegraphics[width=0.75\linewidth]{figures/beta_v.pdf}
\hfill
\caption{Micro-F1 results for classification accuracy on heterophilic nodes ($\beta_v\leq 0.5$). \model{} shows better accuracy on classifying heterophilic nodes than the other methods.}
\label{fig:noisy_neighbours}
\end{figure}


\begin{figure}[t!]
\centering
 \includegraphics[width=0.8\linewidth]{figures/runtime.pdf}
\hfill
\caption{Attention matrix density and training runtime with respect to $k$. Attention matrix sparsified by keeping the top $k$ elements at each row, which effectively improves runtime efficiency.}
\label{fig:density}
\end{figure}


\textbf{Time complexity.} In vanilla \model{}, eigen-decomposition is required for \autoref{eqn:graph_wavelet_matrix} which has a time complexity of $O(N^3)$. \model{}-Cheb and \model{}-ARMA avoid eigen-decomposition and are able to scale to large graphs as their time complexities are $O(R\times|E|)$ and $O((P\times T + Q)\times |E|)$ respectively, where $R$, $P$ and $Q$ are polynomial orders that are normally less than $30$, $T$ is the number of iterations that is normally less than $50$. Therefore, both \model{}-Cheb and \model{}-ARMA scale linearly with the number of edges $|E|$. Readers can refer to \autoref{sec:approximation} for a more detailed introduction of these two methods. Secondly, partial sorting used in the attention sparsification of \autoref{eqn:psi_k} requires $O(N+k \log N)$. Lastly, \autoref{eqn:softmax} is performed on a length-$k$ vector for $N$ rows; therefore, a time complexity of $O(k\times N)$ is needed. In practice, we have $R \sim P \sim T \sim Q \sim k \ll N \ll |E|$ for most graphs, therefore, for a model with $M$ heads, the overall time complexity is $O(M\times R\times|E|)$ for \model{}-Cheb and $O(M \times (P\times T + Q)\times |E|)$ for \model{}-ARMA.

\begin{figure*}[!t]
\centering
 \includegraphics[width=\textwidth]{figures/disassortative_frequenc_ablation.pdf}
\hfill
\caption{Micro-F1 with respect to ablated frequency sub-ranges on heterophilic graphs. We divide the frequency range into a set of sub-ranges with different lengths. The results (a) and (d) reveal the importance of high-frequency range $(1\sim2)$. Further experiments show that there is a subtle difference in the most important range across datasets, but it ranges between $(0.75\sim 1.25)$.}%\q{(this figure is unclear to me: (1) what does "step=XX" mean? (2) what is label for x-axis? (3) we still have space left at the two sides, so can we make the bars in each plot have the same width? (4) the results probably need some further explanation in the above paragraph.)}}
\label{fig:freqency_ablation}
\end{figure*}

% \autoref{table:missing_node_features} summaries classification accuracy with missing node feature ratios ranging from 0\% to 100\%. Our method outperforms all baselines in the \cora graph up to the missing ratio of 90\%. It also performs comparably for the other two datasets. As expected, we see strong robustness in our model again missing feature vectors. In particular, our model improves up the second best model by 4.5\% - 7.9\% for missing rate 50\% - 90\% in \cora, 5.1\% for the missing rate 90\% in \citeseer, and 20\% for the missing 90\% in \pubmed. Unsurprisingly, APPNP, a model with similar flexible feature aggregation capability \citep{DBLP:conf/iclr/KlicperaBG19}, also shows better robustness than the other baselines.

% \begin{table}[t]
% \begin{center}
% \caption{\s{feature dropout in train, validation and test sets} Comparison of node classification accuracy with 0\% to 100\% missing feature vectors. At each missing rate $p$, the feature vectors of $p\%$ randomly chosen nodes are manually set to zero vectors.}
% \scalebox{0.82}{
%  \begin{tabular}{c  c  c  c  c  c  c  c  c  c  c  c  c} 
%  \toprule
%  & & \multicolumn{10}{c}{Accuracy with \% of missing features} \\ \\[-.7em]
%  Dataset & Method & 0 & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90 & 100 \\
%  \midrule
%  \multirow{5}{*}{\cora}
%  & Chebyshev & 79.9 & 80.0 & 79.9 & 77.3 & 79.7 & 76.5 & 79.7 & 77.7 & 76.8 & 76.1 & 71.7 \\
%  & GCN & 81.8 & 81.6 & 79.6 & 78.7 & 78.0 & 75.5 & 75.7 & 74.9 & 69.3 & 61.2 & 53.4 \\
%  & SGC & 81.7 & 80.9 & 80.7 & 79.2 & 79.2 & 77.3 & 78.3 & 77.9 & 75.6 & 76.8 & 73.4 \\
%  & ARMA & 81.8 & 82.9 & 82.0 & 80.2 & 79.4 & 77.6 & 78.1 & 74.8 & 74.3 & 71.1 & 64.9 \\
%  & GAT & 83.1 & 81.8 & 82.2 & 80.7 & 80.9 & 77.7 & 80.5 & 75.9 & 75.9 & 74.4 & 69.9 \\
%  & APPNP & 83.3 & 83.1 & 82.0 & 81.5 & 82.6 & 79.6 & 81.2 & 78.2 & 79.3 & 72.5 & \textbf{73.2} \\
%  & GNAN* & \textbf{84.9} & \textbf{83.3} & \textbf{82.9} & \textbf{81.7} & \textbf{81.3} & \textbf{80.8} & \textbf{80.4} & \textbf{79.2} & \textbf{75.7} & \textbf{69.6} & 6.1 \\
%  \midrule
%  \multirow{5}{*}{\citeseer}
%  & Chebyshev & 68.6 & 69.3 & 67.0 & 66.3 & 58.4 & 63.6 & 59.0 & 54.8 & 53.7 & 53.9 & 51.3 \\
%  & GCN & 70.5 & 70.7 & 70.6 & 71.3 & 65.6 & 68.2 & 63.9 & 64.4 & 62.6 & 59.5 & 54.9 \\
%  & SGC & 71.2 & 71.1 & 71.2 & 70.4 & 67.1 & 70.1 & 67.3 & 64.6 & 65.0 & 61.7 & \textbf{61.7} \\
%  & ARMA & 71.0 & 71.1 & 70.0 & 71.0 & 66.1 & 68.0 & 59.9 & 58.8 & 58.7 & 58.2 & 53.1 \\
%  & GAT & 69.8 & 69.4 & 69.5 & 68.8 & 68.0 & 69.6 & 67.9 & 65.4 & 63.9 & 62.9 & 59.4 \\
%  & APPNP & \textbf{71.6} & \textbf{71.3} & \textbf{70.2} & \textbf{71.6} & \textbf{69.0} & \textbf{70.8} & \textbf{68.1} & \textbf{65.2} & 68.1 & 67.2 & 64.2 \\
%  & GNAN* & 73.0 & 70.8 & 71.6 & 69.5 & 67.5 & 55.5 & 51.9 & 52.2 & 41.6 & 35.6 & 33.6 \\
%  \midrule   
%  \multirow{5}{*}{\pubmed}
%  & Chebyshev & 78.7 & 78.8 & 77.8 & 77.0 & 74.0 & 75.7 & 76.7 & 77.7 & 74.9 & 75.6 & 75.0 \\
%  & GCN & 78.3 & 78.2 & 76.6 & 74.9 & 74.1 & 75.1 & 74.2 & 74.8 & 74.1 & 74.5 & 73.5 \\
%  & SGC & 78.9 & 77.8 & 78.1 & 77.7 & 76.7 & 75.7 & 75.5 & 75.8 & 71.9 & 72.2 & 72.3 \\
%  & ARMA & 78.7 & 76.6 & 77.8 & 77.8 & 75.0 & 77.8 & 77.9 & 77.1 & 76.5 & 76.3 & 76.1 \\
%  & GAT & 78.6 & 78.9 & 78.4 & 78.8 & 78.9 & 76.8 & 78.0 & 76.4 & 76.0 & 75.4 & 74.5 \\
%  & APPNP & \textbf{80.3} & 80.0 & 80.2 & \textbf{78.2} & \textbf{79.5} & \textbf{78.9} & 78.6 & 79.1 & 79.4 & 78.3 & 77.2 \\
%  & GNAN* & 79.6 & 77.7 & 78.0 & 78.0 & \text{77.0} & \textbf{77.1} & \textbf{77.2} & \textbf{75.2} & \textbf{75.0} & \textbf{71.1} & 36.3 \\
%  \bottomrule
% \end{tabular}}
% \label{table:missing_node_features}
% \end{center}
% \end{table}

% \begin{table}[t]
% \begin{center}
% \caption{Comparison of node classification accuracy with 0\% to 100\% missing feature vectors. At each missing rate $p$, the feature vectors of $p\%$ randomly chosen nodes are manually set to zero vectors.}
% \scalebox{0.82}{
%  \begin{tabular}{c  c  c  c  c  c  c  c  c  c  c  c  c} 
%  \toprule
%  & & \multicolumn{10}{c}{Accuracy with \% of missing features} \\ \\[-.7em]
%  Dataset & Method & 0 & 10 & 20 & 30 & 40 & 50 & 60 & 70 & 80 & 90 & 100 \\
%  \midrule
%  \multirow{5}{*}{\cora}
%  & Chebyshev & 80.4 & 80.8 & 79.7 & 78.5 & 77.4 & 76.6 & 72.6 & 64.5 & 62.2 & 41.2 & 14.9 \\
%  & GCN & 81.9 & 81.5 & 80 & 79.1 & 77.9 & 78.4 & 65 & 55.7 & 37.6 & 20.9 & 14.9 \\
%  & SGC & 81.7 & 81.4 & 81.1 & 70.6?? & 79.3 & 78.5 & 74.5 & 70.2 & 65.6 & 51.3 & 14.9 \\
%  & ARMA & 81.4 & 81.9 & 82.1 & 80.1 & 79.7 & 78.8 & 68.8 & 59.9 & 50 & 26.7 & 6.4 \\
%  & GAT & 83.1 & 82.6 & 82.3 & 81.0 & 80.5 & 79.5 & 73.4 & 70.2 & 63 & 45.9 & 31.9 \\
%  & APPNP & 83.3 & 82.5 & 82.2 & 81.2 & 80.9 & 81.5 & 75.1 & 71.3 & 69.1 & 64.6 & \textbf{60.1} \\
%  & GNAN* & \textbf{84.9} & \textbf{83.3} & \textbf{82.9} & \textbf{81.7} & \textbf{81.3} & \textbf{80.8} & \textbf{80.4} & \textbf{79.2} & \textbf{75.7} & \textbf{69.6} & 6.1 \\
%  \midrule
%  \multirow{5}{*}{\citeseer}
%  & Chebyshev & 68.6 & 68.7 & 68 & 67.1 & 64.5 & 59.2 & 52 & 47 & 36.9 & 25.5 & 16.9 \\
%  & GCN & 70.5 & 71.7 & 70.9 & 71.3 & 69.6 & 64.3 & 56 & 43.5 & 27.8 & 22.6 & 16.9 \\
%  & SGC & 71.2 & 70.8 & 70.4 & 69.4 & 68.2 & 65.2 & 61.6 & 58.6 & 51.8 & 38.9 & \textbf{18.2} \\
%  & ARMA & 71.0 & 71.4 & 69.8 & 71.1 & 67.9 & 61.9 & 56.1 & 47.1 & 30.9 & 18.9 & 16 \\
%  & GAT & 70.5 & 69.5 & 69.4 & 68.2 & 68.7 & 64.3 & 57 & 53.9 & 50.4 & 33.8 & 18.1 \\
%  & APPNP & \textbf{71.6} & \textbf{71.9} & \textbf{71.1} & \textbf{72.1} & \textbf{69.9} & \textbf{66} & \textbf{60.9} & \textbf{57.9} & 39.3 & 18.3 & 16.9 \\
%  & GNAN* & 69.2 & 68.5 & 67.8 & 66.9 & 64.5 & 60.9 & 58.5 & 55.4 & \textbf{51.3} & \textbf{44} & 14.9 \\
%  \midrule   
%  \multirow{5}{*}{\pubmed}
%  & Chebyshev & 78.7 & 77.8 & 77.7 & 76.2 & 77.5 & 71.4 & 73.4 & 66.7 & 56.1 & 44.1 & 40.7 \\
%  & GCN & 78.3 & 77.6 & 77.3 & 76.0 & 76.1 & 70.9 & 66.7 & 69.1 & 63.6 & 45 & 40.7 \\
%  & SGC & 78.9 & 78.2 & 78.1 & 77.3 & 78.2 & 73.6 & 72.5 & 68.5 & 58.1 & 43.4 & 40.7 \\
%  & ARMA & 78.7 & 77.9 & 77.5 & 77.2 & 78.2 & 739 & 69.2 & 71.3 & 67.9 & 47 & 40.7 \\
%  & GAT & 78.6 & 78.5 & 78.5 & 78.6 & 78.6 & 73.8 & 69.4 & 61.2 & 47.7 & 40.7 & 40.7 \\
%  & APPNP & \textbf{80.3} & 79.9 & 79.8 & \textbf{79.6} & \textbf{80.0} & \textbf{77.5} & 76.5 & 73.9 & 72.4 & 48.9 & 18 \\
%  & GNAN* & 79.6 & 77.7 & 78.0 & 78.0 & \text{77.0} & \textbf{77.1} & \textbf{77.2} & \textbf{75.2} & \textbf{75.0} & \textbf{71.1} & 36.3 \\
%  \bottomrule
% \end{tabular}}
% \label{table:missing_node_features}
% \end{center}
% \end{table}


==> ASGAT - ArXiv (2)/introduction.tex <==
\section{Introduction}

Graph neural networks (GNNs) have recently demonstrated great power in graph-related learning tasks, such as node classification~\citep{DBLP:conf/iclr/KipfW17}, link prediction~\citep{NIPS2018_7763} and graph classification \citep{DBLP:conf/kdd/LeeRK18}. Most GNNs follow a message-passing architecture where, in each GNN layer, a node aggregates information from its direct neighbors indifferently. In this architecture, information from long-distance nodes is propagated and aggregated by stacking multiple GNN layers together~\citep{DBLP:conf/iclr/KipfW17, DBLP:conf/iclr/VelickovicCCRLB18, DBLP:conf/nips/DefferrardBV16}. However, this architecture underlies the assumption of local homophily, i.e. proximity of similar nodes.
While this assumption seems reasonable and helpful to achieve good prediction results on homophilic graphs such as citation networks~\citep{Pei2020}, it limits GNNs' generalizability to heterophilic graphs. 
Heterophilic graphs commonly exist in the real-world, for instance, people tend to connect to opposite gender in dating networks, and different amino acid types are more likely to form connections in protein structures \citep{DBLP:conf/nips/ZhuYZHAK20}. Moreover, determining whether a graph is homophilic or not is a challenge by itself. In fact, strong and weak homophily can both exhibit in different parts of a graph, which makes a learning task more challenging. 

% \dw{(The second paragraph seems not necessary in introduction. The first sentence of the third paragraph goes well with the last sentence of the first paragraph.)}\q{(I agree with Dongwoo.)}
% Firstly, the role of nodes in Webgraphs (networks of web pages) and graphs in sociology can be defined solely by network structure regardless of node attributes~\citep{Ribeiro2017}, or influenced by both neighboring and distant nodes~\citep{Liu2020}. Secondly, when node features are aggregated equally hop-by-hop, the feature "majority" would have a strong presence in resulting embedding while the "minority" would have less presence. Eventually, as a GNN goes deeper, the node embeddings become indistinguishable (over-smoothed)~\citep{DBLP:conf/aaai/LiHW18, DBLP:conf/iclr/ZhaoA20}. Recent researches try to "break out" the hop-based aggregation using edge dropout~\citep{DBLP:conf/iclr/RongHXH20}, layer skipping ranges~\citep{DBLP:conf/icml/XuLTSKJ18}, teleporting~\citep{DBLP:conf/iclr/KlicperaBG19} and residue connections~\citep{DBLP:conf/iccv/Li0TG19}. These techniques have shown improved performance in deep GNNs. However, the fundamental design of most GNNs still resembles Laplacian smoothing thus the problem is eased rather than mitigated. 

% Although  local discontinuities are treated as noise and discarded even though they may hold important information~\citep{DBLP:journals/spm/ShumanNFOV13}.

\citet{Pei2020} proposed a metric to measure local node homophily based on how many neighbors of a node are from the same class. Using this metric, they categorized graphs as homophilic (strong homophily) or heterophilic (weak homophily), and showed that classical GNNs such as GCN~\citep{DBLP:conf/iclr/KipfW17} and GAT~\citep{DBLP:conf/iclr/VelickovicCCRLB18} perform poorly on heterophilic graphs. \citet{Liu2020} further showed that GCN and GAT are outperformed by a simple multi-layer perceptron (MLP) in node classification tasks on heterophilic graphs. This is because the naive local aggregation of homophilic models brings in more noise than useful information for such graphs. These findings indicate that these GNN models perform sub-optimally when the fundamental assumption of homophily does not hold.

Based on the above observation, we argue that a well-generalized GNN should perform well on graphs regardless of homophily. Furthermore, since a real-world graph can exhibit both strong and weak homophily in different node neighborhoods, a powerful GNN model should be able to aggregate node features using different strategies accordingly. For instance, in heterophilic graphs where a node shares no similarity with any of its direct neighbors, such a GNN model should be able to ignore direct neighbors and reach farther to find similar nodes, or at least, resort to the node's attributes to make a prediction. Since the validity of the assumption about homophily is often unknown, such aggregation strategies should be learned from data rather than decided upfront. 

To circumvent this issue, in this paper, we propose a novel GNN model with attention-based adaptive aggregation, called \model. Most existing attention-based aggregation architectures perform self-attention to the local neighborhood of a node~\citep{DBLP:conf/iclr/VelickovicCCRLB18}. Unlike these approaches, we aim to design an aggregation method that can gather informative features from both close and far-distant nodes. To achieve this, we employ graph wavelets under a relaxed condition of localization, which enables us to learn attention weights for nodes in the spectral domain. In doing so, the model can effectively capture information from frequency components and thus aggregate both local information and global structure into node representations.

To further improve the generalizability of our model, instead of using predefined spectral kernels, we propose to use multi-layer perceptrons (MLP) to learn desired spectral filters without limiting their shapes. Existing works on graph wavelet transform choose wavelet filters heuristically, such as heat kernel, wave kernel and personalized page rank kernel \citep{DBLP:conf/nips/KlicperaWG19,DBLP:conf/iclr/XuSCQC19,DBLP:conf/iclr/KlicperaBG19}. They are mostly low-pass filters, which means that these models implicitly treat high-frequency components as ``noises'' and have them discarded~\citep{DBLP:journals/corr/abs-1905-09550, DBLP:journals/spm/ShumanNFOV13, Hammond2011, DBLP:journals/corr/abs-2003-07450}. However, this may hinder the generalizability of models since high-frequency components can carry meaningful information about local discontinuities, as analyzed in \citep{DBLP:journals/spm/ShumanNFOV13}. Our model overcomes these limitations using node attentions derived from fully learnable spectral filters.

To summarize, the main contributions of this work are as follows:
\begin{enumerate}
  \item We show that high-frequency components carry important information on heterophilic graphs which can be used to improve prediction performance.
  \item We propose a generalized GNN model which performs well on both homophilic and heterophilic graphs, regardless of graph homophily.
  \item We exhibit that multi-headed attention produced by multiple spectral filters work better than attention obtained from a single filter, as it enables flexibility to aggregate features from different frequency components.
\end{enumerate}

%This model with a global self-attention mechanism, called \model, is realized using fully learnable spectral filters, which enables attention weights to be distributed across a graph sparsely. 

We conduct extensive experiments to compare \model{} with well-known baselines on node classification tasks. The experimental results show that \model{} significantly outperforms the state-of-the-art methods on heterophilic graphs where local node homophily is weak, and performs comparably with the state-of-the-art methods on homophilic graphs where local node homophily is strong. This empirically verifies that \model{} is a general model for learning on different types of graphs.
% Following analysis, we observe the learned filters are of various shapes and in contradiction to common choices of low-pass filters, they have a strong composition of high-frequency components which benefits predictions in heterophilic graphs.

==> ASGAT - ArXiv (2)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
%\def\sN{{\mathbb{N}}}
\def\sN{{\mathcal{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> ASGAT - ArXiv (2)/new_method.tex <==
\section{Proposed Approach}

\begin{figure*}[!t]
\centering
\includegraphics[width=0.95\textwidth]{figures/illustration.pdf}
\caption{Illustration of a spectral node attention layer on a three-hop ego network of the central node $v$ from the \citeseer{} dataset. Node classes are indicated by shape and color. Passing the graph through two learned spectral filters place attention scores on nodes, including node $v$ itself. Nodes with positive attention scores are presented in color. Node features are aggregated for node $v$ according to attention scores. The low-pass filter attend to local neighbors (filter 1), while the high-pass filter skips the first hop and attend the nodes in the second hop (filter $K$). The resulting embeddings from multiple heads are then concatenated before being sent to the next layer (multi-head concatenation). Note that we have visualized learned filters from experiments.}
\label{fig:illustration}
\end{figure*}

Graph neural networks (GNNs) learn lower-dimensional embeddings of nodes from graph structured data. In general, given a node, GNNs iteratively aggregate information from its neighbor nodes, and then combine the aggregated information with its own information. An embedding of node $v$ at the $l$th layer of GNN is typically formulated as
\begin{align*}
\vm_v &= \text{aggregate}(\{\vh^{(l-1)}_u | u \in \sN_v \}) \\
\vh^{(l)}_v &= \text{combine}(\vh^{(l-1)}_v, \vm_v),
\end{align*}
where $\sN_v$ is the set of neighbor nodes of node $v$, $\vm_v$ is the aggregated information from the neighbors, and $\vh^{(l)}_v$ is the embedding of node $v$ at the $l$th layer ($\vh^{(0)}_v = \vx_v$). The embedding $\vh^{(L)}_v$ of node $v$ at the final layer is then used for some prediction tasks. In most GNNs, $\sN_v$ is restricted to a set of one-hop neighbors of node $v$. Therefore, one needs to stack multiple aggregation layers in order to collect the information from more than one-hop neighborhood within this architecture.

\textbf{Adaptive spectral filters.} Instead of stacking multiple aggregation layers, we introduce a spectral attention layer that rewires a graph based on spectral graph wavelets. A spectral graph wavelet $\boldsymbol\psi_v$ at node $v$ is a modulation in the spectral domain of signals centered around the node $v$, given by an $N$-dimensional vector
\begin{align}
\boldsymbol\psi_v = \mU g(\Lambda) \mU^{H} \delta_v,
\label{eqn:wavelet}
\end{align}
where $g(\cdot)$ is a spectral filter and $\delta_v$ is a one-hot vector for node $v$.

The common choice of a spectral filter is a heat kernel. A wavelet coefficient $\psi_{vu}$ computed from a heat kernel can be interpreted as the amount of energy that node $v$ has received from node $u$ in its local neighborhood. In this work, instead of using pre-defined localized kernels, we use multi-layer perceptrons (MLP) to learn spectral filters. With learnable spectral kernels, we obtain the inverse graph wavelet transform
\begin{align}\label{eqn:graph_wavelet_matrix}
\boldsymbol\psi_v = \mU \text{diag}(\text{MLP}(\Lambda)) \mU^H \delta_v.
\end{align}

%where MLP is composed of two-hidden layers. 
\noindent Unlike a low-pass heat kernel, where the wavelet coefficients can be understood as the amount of energy after heat diffusion, the learned coeffcients $\psi_{vu}$ do not always correspond to energy diffusion. In spectral imaging processing, lower frequency components preserve an image's background, while higher frequency components are useful to detect object edges or outlines. Similarly, in spectral graph theory, lower-frequency components carry smoothly changing signals. Therefore a low-pass filter is a reasonable choice to extract features and denoise a homophilic graph. In contrary, higher-frequency components carry abruptly changing signals, which correspond to the discontinuities and "opposite attraction" characteristics of heterophilic graphs. Since $\text{MLP}(\Lambda)$ is learned in training, it can learn a low-pass filter which works as a diffusion operator, while in other cases, especially on heterophilic graphs, it converges to a high-pass filer at most times (\autoref{sec:experiments}).

 Note that we use the terminology wavelet and spectral filter interchangeably as we have relaxed the wavelet definition from \citep{Hammond2011} so that learnable spectral filters in our work are not necessarily localized in the spectral and spatial domains.
  \begin{remark}
 \autoref{eqn:graph_wavelet_matrix} requires the eigen-decomposition of a Laplacian matrix, which is expensive and infeasible for large graphs. To address this computational issue, one may use well-studied methods such as Chebyshev~\citep{Hammond2011, DBLP:conf/iclr/XuSCQC19, DBLP:conf/nips/KlicperaWG19} and Auto-Regressive Moving-Average (ARMA)~\citep{Isufi2017, Liu2019} to efficiently compute an approximate the graph filtering of MLP in \autoref{eqn:graph_wavelet_matrix}.
 \end{remark}

 %\textbf{Approximation of graph filtering.} \autoref{eqn:graph_wavelet_matrix} requires the eigen-decomposition of a Laplacian matrix, which is expensive and infeasible for large graphs. Fortunately, the graph filtering operation can be approximated without eigen-decomposition using well-studied methods like Chebyshev~\citep{Hammond2011, DBLP:conf/iclr/XuSCQC19, DBLP:conf/nips/KlicperaWG19}, Lanzcos~\citep{susnjara2015accelerated}, Cayley~\citep{Levie2019}, Auto-Regressive Moving-Average (ARMA) graph filters~\citep{Bianchi2019} and feedback-looped filters~\citep{Wijesinghe2019}. Chebyshev and Lanzcos are both polynomial methods. Chebyshev is the most widely used method because of its efficiency, stability and relatively fewer hyper-parameters. Cayley, ARMA and feedback-looped filters are rational methods that are known for better approximation accuracy~\citep{Isufi2017}. In general, rational methods are less efficient than polynomial method and have more hyper-parameters. \autoref{sec:experiments} shows results from two different implementations with Chebyshev polynomials and ARMA, both methods scales linearly with the number of edges $|E|$ in graph. Details of the two methods are briefly described in \autoref{sec:approximation}.
 % and we briefly discuss \q{how these methods can be formulated as an instance of approximation for graph filtering in our model} in \s{Section ?}. 


% In addition to these, following \citep{DBLP:conf/iclr/XuSCQC19, DBLP:conf/nips/KlicperaWG19}, we use a fast algorithm to efficiently approximate graph wavelet transform, which has computational complexity $O(p\times|E|)$, where $p$ is the order of Chebyshev polynomials and $|E|$ is the number of edges in a graph.

\textbf{Attention mechanism.~}%\textbf{B. Spectral Node Attentions.}  
Unlike the previous work~\citep{DBLP:conf/iclr/XuSCQC19} where the output of inverse graph wavelet transform are directly used to compute node embeddings, we normalize the output through a softmax layer
\begin{align}
\label{eqn:softmax}
\va_v = \text{softmax}(\boldsymbol\psi_v),
\end{align}

\noindent where $\va_v\in \mathbb{R}^N$ is an attention weight vector. With attention weights, an update layer is then formalized as
\begin{align}
\label{eqn:layer}
\vh^{(l)}_v =  \sigma\left(\sum_{u=1}^{N} \eva_{vu} \vh^{(l-1)}_u \mW^{(l)}\right),    
\end{align}
where $\mW^{(l)}$ is a weight matrix shared across all nodes at the $l$th layer and $\sigma$ is ELU nonlinear activation.  
%\dw{(I'm not fully convinced by the following statement. The attention weight can be a result of a certain combination of low frequency and high frequency components via MLP.) In analogy, the attention weight $\eva$ can be understood as a similarity measurement between pixels on a image: if pixel $v$ is in a homophilic neighbourhood, $\eva$ would be large for its neighbours $u\in N$; if pixel $v$ is an "edge pixel", $\eva$ would be large for another pixel $u$ on the same "edge".}

Note that the update layer is not divided into aggregation and combine steps in our work. Instead, we compute the attention $\eva_{vv}$ directly from a spectral filter. Unlike heat kernel and other spectral filters, the output of inverse graph wavelet transform with a learnable spectral kernel are not always localized. Hence, the model can adaptively aggregate information from both close and far-distant nodes, depending on their attention weights.



\textbf{Sparsified node attentions.} %\q{this subheading is too similar to the previous one. can we change it to something different}
With predefined localized spectral filters such as a heat kernel, most of wavelet coefficients are zero due to their locality. In our work, spectral filters are fully learned from data, consequently attention weights obtained from learnable spectral filters do not impose any sparsity. This means that to perform an aggregation operation we need to retrieve all possible nodes in a graph, which is not efficient. From our experiments, we observe that most attention weights are negligible after softmax. %\To sparsify attention weights, 
Thus, we consider a sparsification technique to keep only the largest $k$ entries of \autoref{eqn:graph_wavelet_matrix} for each node, i.e.
  \begin{align}
        \label{eqn:psi_k}
        \bar{{\psi}}_{vu} = 
        \begin{cases} 
            {\psi}_{vu} & \quad \text{ if } {\psi}_{vu} \in \text{topK}(\{\psi_{v0}, ..., \psi_{vN}\}, k) \\
            -\infty & \quad \text{ otherwise},
        \end{cases}
    \end{align}
where topK is a partial sorting function that returns the largest $k$ entries from a set of wavelet bases $\{\psi_{v0}, ..., \psi_{vN}\}$. This technique guarantees attention sparsity such that the embedding of each node can be aggregated from at most $k$ other nodes with a time complexity trade-off of $O(N+k\log N)$.
The resulting $\bar{\psi}$ is then fed into the softmax layer to compute attention weights.

We adopt multi-head attention to model multiple spectral filters. Each attention head aggregates node information with a different spectral filter, and the aggregated embedding is concatenated before sent to the next layer. 
To reduce redundancy, we adopt a single MLP$:\sR^N \rightarrow \sR^{N\times M}$, where $M$ is the number of attention heads, and each column of the output corresponds to one adaptive spectral filter.
%\s{\sout{An option is using independent MLPs for each filter. However, in practice, we found the independent MLPs turn to converge to similar shapes. thus introduce redundancy and increase computational complexity. Therefore, we adopt a singpe MLP with fixed-dimensional output, each corresponding to one adaptive spectral filter.}}

We name the multi-head spectral attention architecture as a \emph{adaptive spectral graph attention network} (\model{}). The design of \model{} is easily generalizable, and many existing GNNs can be expressed as special cases of \model{} (see \autoref{sec:connection}). \autoref{fig:illustration} illustrates how \model{} works with two attention heads learned from the \citeseer{} dataset. As shown in the illustration, the MLP learns adaptive filters such as low-pass and high-pass filters. A low-pass filter assigns high attention weights in local neighborhoods, while a high-pass filter assigns high attention weights on far-distant but similar nodes, which cannot be captured by a traditional hop-by-hop aggregation scheme.

%\dw{What is the computational complexity of the model? Do we have any trick used to reduce it other than the polynomial approximation?}




==> ASGAT - ArXiv (2)/preliminaries.tex <==
\section{Preliminaries}

%We start by providing some related background with useful notations. 

%\subsection{Spectral Graph Filters And Wavelets}

% Similar to decimation in the classical signal processing, graph decimation aims to sample a subset of nodes $\mathcal{S} \subset V$ where $|\mathcal{S}| \ll |V|$ such that the graph signal $\hat{\boldsymbol{x}}$ reconstructed from $S$ is a close approximation of $\boldsymbol{x}$~\citep{DBLP:conf/icassp/NarangO11}.

% Graph decimation is normally performed in the spectral domain for better generalization and nice theoretical characteristics~\citep{DBLP:journals/tsp/SakiyamaTTO19, DBLP:journals/tsp/Tanaka18, DBLP:journals/corr/abs-1711-02046, DBLP:journals/corr/PuyTGV15}. Spectral graph decimation is also often seen in literature related to graph multi-scale analysis \citep{DBLP:journals/corr/abs-1711-02046}. Graph decimation applies multiple low-pass and high-pass filters iteratively to form a cascaded filter bank which outputs coarsen graphs at different scales. In this paper, due to page limit, we use graph decimation as a node sampling method and do not explore the its application in multi-scale analysis.

Let $\gG=(V,E,A, \boldsymbol{x})$ be an undirected graph with $N$ nodes, where $V$, $E$, and $A$ are the node set, edge set, and adjacency matrix of $\gG$, respectively, and $\boldsymbol{x}: V\mapsto \mathbb{R}^m$ is a graph signal function that associates each node with a feature vector. The normalized Laplacian matrix of $\gG$ is defined as $\mL = \mI - \mD^{-1/2}\mA\mD^{-1/2}$, where $\mD \in {\mathbb R}^{N\times N}$ is the diagonal degree matrix of $\gG$. 
%\q{\sout{$A$ is the adjacency matrix.} ($A$ has already been defined above)} 
In spectral graph theory, the eigenvalues $\Lambda = \text{diag}(\lambda_1,...,\lambda_N)$ and eigenvectors $\mU$ of $\mL = \mU\Lambda \mU^H$ are known as the graph's spectrum and spectral basis, respectively, where $\mU^H$ is the Hermitian transpose of $\mU$. The graph Fourier transform of $\boldsymbol{x}$ is $\boldsymbol{\hat{x}} = \mU^H\boldsymbol{x}$ and its inverse is $\boldsymbol{x} = \mU\hat{\boldsymbol{x}}$.

The spectrum and spectral basis carry important information on the connectivity of a graph~\citep{DBLP:journals/spm/ShumanNFOV13}. Intuitively, lower frequencies correspond to global and smooth information on the graph, while higher frequencies correspond to local information, discontinuities and possible noise~\citep{DBLP:journals/spm/ShumanNFOV13}. One can apply a spectral filter and use graph Fourier transform to manipulate signals on a graph in various ways, such as smoothing and denoising~\citep{DBLP:conf/globalsip/SchaubS18}, abnormally detection~\citep{5967745} and clustering~\citep{8462239}.
Spectral convolution on graphs is defined as the multiplication of a signal $\vx$ with a filter $g(\Lambda)$ in the Fourier domain, i.e.
\begin{equation}\label{eqn:spectral_filter}
g(\mL)\vec{x} = g(\mU\Lambda \mU^H)\vec{x} = \mU g(\Lambda)\mU^H\vec{x} = \mU g(\Lambda)\hat{\vec{x}}.
\end{equation}
When a spectral filter is parameterized by a scale factor, which controls the radius of neighbourhood aggregation, \autoref{eqn:spectral_filter} is also known as the Spectral Graph Wavelet Transform (SGWT)~\citep{Hammond2011, DBLP:journals/spm/ShumanNFOV13}. For example, \citet{DBLP:conf/iclr/XuSCQC19} uses a small scale parameter $s < 2$ for a heat kernel, $g(s\lambda) = e^{-\lambda s}$, to localize the wavelet at a node. 

%where a filter is often chosen heuristically, such as heat kernel, wave kernel and personalized page rank kernel~\citep{DBLP:conf/nips/KlicperaWG19}.

==> ASGAT - ArXiv (2)/related_work.tex <==
\section{Related Work}
\label{related_work}
%Now we discuss the related work and show how our approach differs from existing work.

%\subsection{Graph Attention Mechanism}

Graph neural networks have been extensively studied recently. We categorize work relevant to ours into three perspectives and summarize the key ideas.

\textbf{Attention on graphs.} 
%Self-attention mechanism has been actively researched in both language and vision models because it can simultaneously capture local and long-distance dependency. While self-attention was first proposed as a language model which has shown greater performance over recurrent neural network models \citep{DBLP:conf/nips/VaswaniSPUJGKP17}, it has also been transplanted successfully in the field of vision. Recent studies \citep{DBLP:conf/iclr/CordonnierLJ20, DBLP:conf/nips/ParmarRVBLS19} show attention layers can effectively learn, but not limited to, convolutional operations on images. In another word, with sufficient number of heads, attention layers can be at least as expressive as any convolutional and recurrent layers.
Graph attention networks (GAT) \citep{DBLP:conf/iclr/VelickovicCCRLB18} was the first to introduce attention mechanisms on graphs. GAT assigns different importance scores to local neighbors via an attention mechanism. Similar to other GNN variants, long-distance information propagation in GAT is realized by stacking multiple layers together. Therefore, GAT suffers from the oversmoothing issue \citep{DBLP:conf/iclr/ZhaoA20}. 
%Instead of using only one-hop neighbours, we argue that graph attentions benefit from aggregation schemes within adaptive neighbourhoods. However, in contrast to self-attention on regular data, self-attention on graphs should respect a graph's topology and connectivity and behave under such constraints. Also, pair-wise attention weights for all nodes are expensive to computed especially for large graphs. There the graph attention mechanism should attend nodes selectively for efficiency.
%To the best of our knowledge, \citet{DBLP:conf/iclr/VelickovicCCRLB18} are the first to apply attention mechanism on graphs (GAT). 
\citet{DBLP:conf/iclr/0001ZWZ20} improve GAT by incorporating both structural and feature similarities while computing attention scores.

\textbf{Spectral graph filters and wavelets.} Some GNNs also use graph wavelets to extract information from graphs. \citet{DBLP:conf/iclr/XuSCQC19} applied graph wavelet transform defined by \citet{DBLP:journals/spm/ShumanNFOV13} to GNNs. \citet{DBLP:conf/nips/KlicperaWG19} proposed a general GNN argumentation using graph diffusion kernels to rewire the nodes. \citet{DBLP:conf/kdd/DonnatZHL18} used heat wavelet to learn node embeddings in unsupervised ways and showed that the learned embeddings closely capture structural similarities between nodes. Other spectral filters used in GNNs can also be viewed as special forms of graph wavelets~\citep{DBLP:conf/iclr/KipfW17, DBLP:conf/nips/DefferrardBV16, DBLP:journals/corr/abs-1901-01343}. Coincidentally, \citet{DBLP:journals/corr/abs-2003-07450} also noticed useful information carried by high-frequency components from a graph Laplacian. Similarly, they attempted to utilize such components using node attentions. However, they resorted to the traditional choice of heat kernels and applied such kernels separately to low-frequency and high-frequency components divided by a hyperparameter. In addition to this, their work did not link high-frequency components to heterophilic graphs.

\textbf{Prediction on heterophilic graphs.} \citet{Pei2020} have drawn attention to GCN and GAT's poor performance on heterophilic graphs very recently. They try to address the issue by essentially pivoting feature aggregation to structural neighborhoods from a continuous latent space learned by unsupervised methods. Another attempt to address the issue was proposed by \citet{Liu2020}. They proposed to sort locally aggregated node embeddings along a one-dimensional space and used a one-dimensional convolution layer to aggregate embeddings a second time. By doing so, non-local but similar nodes can be attended to. Very recently, \citet{DBLP:conf/nips/ZhuYZHAK20} showed a heuristic combination of ego-, neighbor and higher-order embedding improves GNN performance on heterophilic graphs. Coincidentally, they also briefly mentioned the importance of higher-frequency components on heterophilic graphs, but they did not provide an empirical analysis.

Although our method shares some similarities in motivation with the aforementioned work, it is fundamentally different in several aspects. To the best of our knowledge, our method is the first architecture we know that computes multi-headed node attention weights purely from learned spectral filters. As a result, in contrast to commonly used heat kernel, our method utilizes higher-frequency components of a graph, which helps prediction on heterophilic graphs and neighbourhoods.


==> ASGAT - ArXiv (2)/relationships.tex <==
\section{Connections to Other Methods}
\label{sec:connection}

In this section, we show \model{} has strong connection to existing models, and many GNNs can be expressed as a special case of \model{} under certain conditions.

\subsection{Connection to GCN}

A GCN~\citep{DBLP:conf/iclr/KipfW17} layer can be expressed as

$$\vh_v^{(l)} = \operatorname{ReLU}(\sum^N_{u=1}\hat{a}_{vu}\vh_u^{(l-1)}\mW^{(l)})$$

where $\hat{a}_{vu}$ is the elements from the $v$-th row of the symmetric adjacency matrix

$$\hat{\mA}=\tilde{\mD}^{-1/2}\tilde{\mA}\tilde{\mD}^{-1/2}  \quad
\text{where} \quad \tilde{A} = \mA + \mI_N,\; \tilde{\emD}_{vv} = \sum_{u=1}^N\tilde{\emA}_{vu}$$

So that

$$
\hat{a}_{vu} = \begin{cases} 1 & \text{if} \; e_{vu} \in E \\ 0 & if \; e_{vu} \notin E\end{cases}
$$

Therefore, GCN can be viewed as a case of \autoref{eqn:layer} with $\sigma = \operatorname{ReLU}$ and $a_{vu} = \hat{a}_{vu}$

\subsection{Connection to Polynomial Filters}

Polynomial filters localize in a node's $K$-hop neighbors utilizing $K$-order polynomials~\citep{DBLP:conf/nips/DefferrardBV16}, most of them takes the following form:

$$g_\theta(\Lambda) = \sum^{K-1}_{k=0}\theta_k\Lambda^k$$

where $\theta_k$ is a learnable polynomial coefficient for each order. Thus a GNN layer using a polynomial filter becomes

$$\vh^{(l)}_v=\operatorname{ReLU}(\sum_{u=1}^N \mU g_\theta(\Lambda)\mU^T\vh_u^(l-1))$$

which can be expressed using \autoref{eqn:layer} with $\mW^{(k)} = \mI_N$, $\sigma = \operatorname{ReLU}$ and $a_{vu}=(\mU g_\theta(\Lambda)\mU^T)_{vu}$. In comparison, our method uses a MLP to learn the spectral filters instead of using a polynomial filter. Also, our method introduces an attention mechanism on top of the filtering response.

\subsection{Connection to GAT}

Our method is inspired by and closely related to GAT~\citep{DBLP:conf/iclr/VelickovicCCRLB18}. To demonstrate the connection, we firstly define a matrix $\Phi$ where each column $\bm{\phi}_v$ is the transformed feature vector of node $v$ concatenated with feature vector of another node (including node $v$ itself) in the graph.
\begin{equation}
    \bm{\phi}_v^{(l)} = ||_{j=0}^N [\mW\vh_v^{(l-1)}||\mW\vh_u^{(l-1)}],
\end{equation}
where $\mW$ is a shared weight matrix, $h_v^{(l-1)}$ and $h_u^{(l-1)}$ are the representation for node $v$ and $u$ from the layer $l-1$. GAT multiplies each column of $\Phi$ with a learnable weight vector $\bm{\alpha}$ and masks the result with the adjacency $\mA$ before feeding it to the nonlinear function $\operatorname{LeakyRelu}$ and $\operatorname{softmax}$ to calculate attention scores. The masking can be expressed as a Hadamard product with the adjacency matrix $\mA$ which is the congruent of a graph wavelet transform with the filter $g(\Lambda) = \mI - \Lambda$:
\begin{equation}
    \Psi = \mA = \mD^{\frac{1}{2}}\mU(\mI - \Lambda)\mU^T \mD^{\frac{1}{2}}
\end{equation}
The GAT attention vector for node $v$ becomes
\begin{equation}
    \va_v = \operatorname{softmax}(\operatorname{LeakyReLU}(\bm{\alpha}^T\bm{\phi}_v \odot \bm{\bar{\psi}}_v))
\end{equation}
where $\bm{\bar{\psi}}_v$ is the $v$-th row of $\Psi$, $\odot$ denotes the Hadamard product, as in \citet{DBLP:conf/iclr/VelickovicCCRLB18}.

In comparison with our method, GAT incorporates node features in the attention score calculation, while node attentions in our methods are purely computed from the graph wavelet transform. Attentions in GAT are restricted to node $v$'s one-hop neighbours only.

\subsection{Connection to Skip-gram methods}

Skip-gram models in natural language processing are shown to be equivalent to a form of matrix factorization \citep{DBLP:conf/nips/LevyG14}. Recently \citet{DBLP:conf/wsdm/QiuDMLWT18} proved that many Skip-Gram Negative Sampling (SGNS) models used in node embedding, including DeepWalk~\citep{DBLP:conf/kdd/PerozziAS14}, LINE~\citep{DBLP:conf/www/TangQWZYM15}, PTE~\citep{DBLP:conf/kdd/TangQM15}, and node2vec~\citep{DBLP:conf/kdd/GroverL16}, are essentially factorizing implicit matrices closely related to the normalized graph Laplacian. The implicit matrices can be presented as graph wavelet transforms on the normalized graph Laplacian. For simplicity, we use DeepWalk, a generalized form of LINE and PTE, as an example. \citet{DBLP:conf/wsdm/QiuDMLWT18} shows DeepWalk effectively factorizes the matrix
\begin{equation}
\label{eqn:SGNS_matrix}
\log\left(\frac{\operatorname{vol}(\gG)}{K}(\sum_{r=1}^K\mP^r)\mD^{-1}\right)-\log(b)
\end{equation}
where $\operatorname{vol}(\gG) =\sum_v \emD_{vv}$ is the sum of node degrees, $\mP=\mD^{-1}\mA$ is the random walk matrix, $K$ is the skip-gram window size (number of hops) and $b$ is the parameter for negative sampling. We know that
$$
\mP = \mI - \mD^{-\frac{1}{2}}\mL\mD^{\frac{1}{2}} = \mD^{-\frac{1}{2}}\mU(\mI - \Lambda)\mU^T\mD^{\frac{1}{2}}.
$$
So \autoref{eqn:SGNS_matrix} can be written using normalized graph Laplacian as:
$$
\log\left(\frac{\operatorname{vol}(\gG)}{K}\mD^{-\frac{1}{2}}\sum_{r=1}^K(\mI-\mL)^r\mD^{\frac{1}{2}}\right) - \log(b).
$$
Or, after eigen-decomposition, as:
\begin{equation}\label{DeepWalkMatrix}
\mM = \log\left(\frac{\operatorname{vol}(\gG)}{Tb}\mD^{-\frac{1}{2}}\mU\sum_{r=1}^K(\mI-\Lambda)^r\mU^T\mD^{\frac{1}{2}}\right),
\end{equation}
where $\mU\sum_{r=1}^T(\mI-\Lambda)^r\mU^T$, denoted as $\bm{\psi}_{sg}$, is a wavelet transform with the filter $g_{sg}(\lambda) = \sum_{r=1}^K(1 - \lambda)^r$. Therefore, DeepWalk can be seen a special case of \model{} by substituting MLP in \autoref{eqn:graph_wavelet_matrix} with $g_{sg}$, and $a_vu$ in \autoref{eqn:layer} with
\begin{align*}
    \bm{a}_{vu} = 
    \begin{cases} 
        {\psi}_{vu} & \quad \text{ if } d_{vu} \leq K \\
        0 & \quad \text{ if } otherwise
    \end{cases}
\end{align*}
where $d_{vu}$ is the shortest distance between node $v$ and $u$. Assigning $\mH = \mW =\mI$, $K=1$ and $\sigma(X)=\log(\frac{\operatorname{vol}(\gG)}{Tb}\mD^{-\frac{1}{2}}\mX\mD^{\frac{1}{2}})$. We have
\begin{equation}
    \vh'_v=\operatorname{FACTORIZE}(\sigma(\bm{a_v}))
\end{equation}
where $\operatorname{FACTORIZE}$ is a matrix factorization operator of choice. \citet{DBLP:conf/wsdm/QiuDMLWT18} uses SVD in a generalized SGNS model, where  the decomposed matrix $\mU'$ and $\bm\Sigma'$ from $\mM=\mU'\bm\Sigma' \mV'$ is used to obtain the node embedding $\vh_v = \mU'\sqrt{\bm\Sigma'}$.

==> impact.tex <==
% \section*{Impact}

% Authors are required to include a statement of the broader impact of their work, including its ethical aspects and future societal consequences. 
% Authors should discuss both positive and negative outcomes, if any. For instance, authors should discuss a) 
% who may benefit from this research, b) who may be put at disadvantage from this research, c) what are the consequences of failure of the system, and d) whether the task/method leverages
% biases in the data. If authors believe this is not applicable to them, authors can simply state this.

% Use unnumbered first level headings for this section, which should go at the end of the paper. {\bf Note that this section does not count towards the eight pages of content that are allowed.}


% \begin{ack}
% Use unnumbered first level headings for the acknowledgments. All acknowledgments
% go at the end of the paper before the list of references. Moreover, you are required to declare 
% funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work). 
% More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2020/PaperInformation/FundingDisclosure}.

% Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
% \end{ack}

==> method.tex <==
\section{Proposed Method}
\label{sec:methods}
\q{(maybe change the section title to: ``Global Node Attention Networks" or ``Proposed Method", or ...)}

\dw{(there might be a better way to organize this section. let me think about it...)}\q{(That would be great ... I feel the current way is unclear about the whole picture :-))}

In this section, we introduce our proposed method: Global Node Attention Networks (\model), which is a multi-layer neural network. We start by describing a \emph{global node attention layer}, which is a basic building block of \model. Then, we explain how attention scores are computed using \emph{learnable spectral filters} specially designed in our method... \q{adaptive filterbanks in each layer. (this sentence needs some revision later.)}


\begin{figure}[!t]
\centering
\includegraphics[width=1\textwidth]{figures/illustration_new.pdf}
\caption{Illustration of spectral node attention on a 3-hop ego network of the central node $i$ from the \citeseer{} dataset (left). Node classes are indicated by shape and color. Passing the graph through four learned spectral filters (second left) creates four rewired graphs (second right), from each node features, are aggregated for node $i$ (right most). Dashed lines indicate the rewired network. Low-pass filters attend to local neighbors evenly (first and third row), high-pass filters skip hops (second row) or attend to node $i$ itself only (last row). \dw{Maybe, we can send the whole figure to the appendix and use only one (or two) filter in the main text?} \q{I'm also thinking about how to improve/use this figure...maybe: one option is to use part of the figure in the main body as Dongwoo suggests, and another option is to improve this figure and use it to illustrate the key components in an attention layer.}}
\label{fig:illustration}
\end{figure}

\subsection{Global Node Attention Layer}

%We first start by describing a \emph{global node attention layer}, which is a basic building block of GNAN. 

Each global node attention layer consists of $K$ self-attention heads. The input of each self-attention head is a set of node representations, $\{\boldsymbol{h}_i\}_{i=1}^{N}$, where $N=|V|$ is the number of nodes. The node representation $\boldsymbol{h}_i$ of node $i$ is the output of the previous layer if the current layer is not the first layer, otherwise $\boldsymbol{h}_i = \boldsymbol{x}_i$, where $\boldsymbol{x}_i$ is the input feature of node $i$.
 

%For each attention head $k$, we apply a linear transform, parameterized by weight matrix $W$, to all input representation $\vec{h}_j$. The weight matrix $W$ is shared across all nodes and heads $k$. As the next step, we perform a self-attention on the nodes. We defer the detailed explanation on the exact computation of attention score until the next section. For each node $i$, the transformed representation $\boldsymbol{h}_jW$ is aggregated by attention score $\vec{a}_i$, i.e. $\sum_{j=1}^{N} a_{ij}=1$, and then passed through the non-linear activation function $\sigma$. We use ELU non-linear function in out experiments. Finally, we concatenate learned representations from the multiple heads, yielding the following representation for node $i$:
For each self-attention head $k$, we apply a linear transform, parameterized by a weight matrix $W$, to all node representations $\vec{h}_j$ in the input. The weight matrix $W$ is shared across all nodes and self-attention heads. Then, we perform a self-attention on the nodes. We defer the detailed explanation on the exact computation of attention scores until the next section. For each target node $i$, \q{the transformed representation $\boldsymbol{h}_jW$ is (unclear here)} aggregated by an attention \q{vector(?) $\vec{a}_i$, i.e. $\sum_{j=1}^{N} a_{ij}=1$, which contains global node attention scores w.r.t. the node $i$,} and then passed through a non-linear activation function $\sigma$. We use ELU activation function \citep{clevert2015fast} in out experiments. Finally, we concatenate learned representations from all $K$ self-attention heads, yielding the following representation for node $i$:
\begin{equation}
    \label{eqn:layer}
    \boldsymbol{h}'_i = {\Big|\Big|}^K_{k=1} \sigma\big(\sum_{j=1}^{N}{a}_{ij}^{k}\boldsymbol{h}_jW\big),
\end{equation}
where $||$ denotes concatenation operation, $\vec{h}'_i$ is the concatenated representation of node $i$ and is fed into the next layer if any.

\subsection{Spectral Node Attentions}
%To compute the attention score $\vec{a}$, we propose a \emph{learnable spectral filter}. 
Most of the existing attention-based aggregation architectures perform self-attention on the local neighborhood of the current node~\citep{DBLP:conf/iclr/VelickovicCCRLB18}. One thus needs to stack multiple aggregation layers to collect the information from more than one-hop neighborhood with this structure. To alleviate this limitation, we employ graph wavelets and relax the wavelet definition from \citep{Hammond2011} so that they do not have to be localized in the spectral domain. As a result, the computed attention scores can be freely distributed across all nodes.
Formally, a graph wavelet localized at node $i$ is defined as
\begin{align}
    \label{eqn:graph_wavelet}
    \boldsymbol{\psi}_i = Ug(\Lambda)U^H \boldsymbol{\delta_{i}},
\end{align}
where $g(\Lambda)$ is a wavelet kernel, $\boldsymbol{\delta_{i}} = [\delta_{i1},\delta_{i2},...,\delta_{iN}]$ is a Kronecker delta, i.e. $\delta_{ij} = [i=j]$. The resulting $\boldsymbol{\psi}_i$ is the inverse wavelet transform localized at node $i$. Instead of using graph wavelet transform to compute node representations directly \citep{DBLP:conf/kdd/DonnatZHL18, DBLP:conf/iclr/XuSCQC19} in a convolutional setting, we employ these wavelets for computing graph structural node attention scores by applying a \textit{softmax} function. Hence, attention scores are positive and normalized.

\dw{(BTW, in \cite{DBLP:conf/kdd/DonnatZHL18}, the authors prove that two nodes $u$ and $v$ have similar structure if the distribution of $\psi_u$ and $\psi_v$ are similar (although their order in the vectors should not be the same). If this is the case, then we could directly apply the self-attention with permutation invariant function on top of $\psi_u$ and $\psi_v$ to capture their structural similarity?)}


One downside of a fully learned kernel is that it could place attentions densely on the graph which increases computational cost for aggregation. Thus, for better computational efficiency, we sparsify attention scores by discarding the entries of wavelet bases that are below a threshold $t$, i.e.
\begin{align}
\label{eqn:psi}
    \bar{{\psi}}_{ij} = 
    \begin{cases} 
        {\psi}_{ij} & \quad \text{ if } {\psi}_{ij} > t \\
        -\infty & \quad \text{ if } {\psi}_{ij} \leq t
    \end{cases}
\end{align}

Given a sparsified and localized wavelet $\bar{\boldsymbol{\psi}}_i = [\bar{\psi}_{i1},...,\bar{\psi}_{iN}]$, we define attention scores as
\begin{align*}
    \boldsymbol{a}_i = \operatorname{softmax}(
        \bar{\boldsymbol{\psi}}_i
    )
\end{align*}
Therefore, the attention score on node $j$ is zero if $\psi_{ij}$ is less than the given threshold $t$. In our experiments, we set $t = 0$.

\subsection{Adaptive Filters}

Most of the existing work based on graph wavelet transform choose wavelet filters heuristically, such as heat kernel, wave kernel and personalized page rank kernel \citep{DBLP:conf/nips/KlicperaWG19,DBLP:conf/iclr/XuSCQC19,DBLP:conf/iclr/KlicperaBG19}. Some of them also use a separate scale hyperparameter to control the radius of neighbourhood aggregation. For example, \citep{DBLP:conf/iclr/XuSCQC19} uses a small scale parameter $s < 2$ for a heat kernel, $g(s\lambda) = e^{-\lambda s}$, to localize a wavelet at node. While these filters have intuitive interpretations related to diffusion processes~\citep{DBLP:conf/nips/KlicperaWG19}, they implicitly assume local homophily. However, as we will discuss in \autoref{sec:experiments}, this assumption does not hold for some graphs. Another assumption underlying these filters is that high frequencies are "noises" and should be discarded~\citep{DBLP:journals/spm/ShumanNFOV13, Hammond2011, DBLP:journals/corr/abs-2003-07450}.  This assumption is reflected in the heavy use of low-pass filters which discard high-frequency components. Nevertheless, as analyzed in \citep{DBLP:journals/spm/ShumanNFOV13}, high frequencies are not necessarily noises and may carry meaningful information about local discontinuities. We believe the aforementioned assumptions are overly simplistic and rigid. Therefore, we propose to use multi-layer perceptrons (MLP) to learn desired filters without limiting their shapes.

\q{While each attention head could learn wavelet kernels through separate MLPs, in practice, (It's unclear)} we find most kernels tend to converge to filters of similar shape, which increases redundancy and computational cost. Instead, we find it more efficient to use a single MLP with $K$-dimensional outputs, each corresponding to one attention head. So the matrix form of \autoref{eqn:graph_wavelet} becomes
\begin{equation}
    \label{eqn:graph_wavelet_matrix}
    \boldsymbol{\Phi} = U (\text{MLP}(\Lambda)) U^H\Delta
\end{equation}
where $\Delta$ is the Kronecker delta signal in matrix form, i.e. an identity matrix.

% Furthermore, to avoid training cold start, we pre-train the MLP to approximate a $H$-bank itersine filter. The itersine filter equally divide the spectrum into $H$ evenly passing bands. 

\autoref{eqn:graph_wavelet_matrix} requires the eigendecomposition of a Laplacian matrix, which is expensive and infeasible for large graphs. We follow  \citet{DBLP:conf/iclr/XuSCQC19, DBLP:conf/nips/KlicperaWG19} to apprximate graph wavelet transform using Chebyshev Polynomials~\citep{DBLP:journals/spm/ShumanNFOV13}.

